Cross-Coupled Iterative Learning Control for Complex Systems: A Monotonically Convergent and Computationally Efficient Approach

Cross-coupled iterative learning control (ILC) can achieve high performance for manufacturing applications in which tracking a contour is essential for the quality of a product. The aim of this paper is to develop a framework for norm-optimal cross-coupled ILC that enables the use of exact contour errors that are calculated offline, and iteration- and time-varying weights. Conditions for the monotonic convergence of this iteration-varying ILC algorithm are developed. In addition, a resource-efficient implementation is proposed in which the ILC update law is reframed as a linear quadratic tracking problem, reducing the computational load significantly. The approach is illustrated on a simulation example.

==> implementation.tex <==

Regarding the implementation, two aspects are considered. First, a resource-efficient implementation is proposed that reduces the computational load significantly for the ILC algorithm proposed in Section \ref{sec:approach}. This allows for long reference signals and is especially useful when an iteration-varying cost function is used. Secondly, it is observed that the cross-coupled ILC framework leads to an inferential ILC configuration in which feedforward and feedback control actions might oppose each other, and serial ILC is proposed as a solution.

\subsection{Resource-efficient implementation}

To calculate feedforward update $f_{j+1}$ according to (\ref{eq:f_update}) the iteration-varying norm-optimal ILC algorithm is rewritten to a linear quadratic tracking (LQT) problem. As a result, the matrices $Q_j$ and $L_j$ do not have to be calculated explicitly, avoiding the inversion in (\ref{eq:filters}) that would otherwise limit the size of the matrices of the lifted system and thus also the length of the reference signals.

The closed-loop system $J$ that is written in lifted form in the previous sections, is now rewritten to the state-space description given by  
\begin{align}
	\textbf{J}(k) = \left[\begin{array}{c|c} 
		A(k) & B(k)\\ 
		\hline 
		C(k) & D(k) 
	\end{array}\right]. 
\end{align}
In addition, due to the block-diagonal structure of $W_{ec,j}$, $W_{fc,j}$ and $W_{\Delta fc,j}$ the cost function (\ref{eq:cost2}) can be written as
\begin{align} \label{eq:cost3}
	\mathcal{J}(f_{j+1}) = \sum_{k=1}^{N} &\|e_{j+1}(k)\|^2_{W^k_{ec,j}} +  \|f_{j+1}(k)\|_{W^N_{fc,j}}  \\ \nonumber &+ \|f_{j+1}(k) - f_j(k)\|_{W^k_{\Delta fc,j}}, 
\end{align}
where, consistent with the previous notation, $W^k_{ec,j} = (C^k_{e,j})\tran W^k_{e,j} C^k_{e,j}$ etc. In addition, $\Delta f_{j+1}(k) = f_{j+1}(k) - f_j(k)$ and $\Delta x_{j+1}(k) = x_{j+1}(k) - x_j(k)$ are defined. This leads to the following lemma for the optimal input $f_{j+1}$. \rev{omschrijven ejplus1}

\begin{lem}
	The optimal ILC input that minimizes (\ref{eq:cost2}) is the solution to the linear quadratic tracking (LQT) problem with dynamics
	\begin{align}
	\Delta x_{j+1}(k+1) &= A(k) \Delta x_{j+1}(k) + B(k) \Delta f_{j+1}(k) \\ \nonumber
	\Delta y_{j+1}(k) &= C(k)\Delta x_{j+1}(k) + D(k) \Delta f_{j+1}(k),
	\end{align} 
	and cost function \rev{omdraaien}
	\begin{align} \nonumber
		\mathcal{J}&(\Delta f_{j+1}) = \sum_{k=1}^{N} \|\Delta y_j(k) - e_j(k)\|_{W^k_{ec,j}} \\ 
		&+  \|\Delta f_j(k) + f_{j}(k)\|_{W^N_{fc,j}} + \|\Delta f_j(k)\|_{W^k_{\Delta fc,j}}. 
	\end{align}
\end{lem}

The approach to solving discrete-time LQT problems is well-known and described in, e.g., \cite[Section 4.4]{Lewis2012}. The approach consists of defining a Hamiltonian system, leading to a two-point boundary value problem, to which a sweep method is applied that involves solving part of the equations backwards in time. For the cross-coupled ILC problem this leads to the following solution. For ease of notation, the time indices $(k)$ for the LTV system $\textbf{J}_j^{ILC}(k)$ and time-varying system matrices such as $A(k)$ and $L_j(k)$ are omitted in most equations.
\begin{align}
	f_{j+1}(k) = \textbf{J}_j^{ILC}(k) \begin{bmatrix} e_j(k) \tran & f_j(k)  \tran & g_j(k+1)\tran \end{bmatrix} \tran,
\end{align}
with
\begin{align}
	\textbf{J}_j^{ILC}	&= 
	\left[\begin{array}{c|ccc} 
		A - B L_j & B L_{ec,j} & -B L_{fc,j} & B L_{g,j}\\ 
		\hline 
		-L_j & L_{ec,j} & I-L_{fc,j} & L_{g,j} 
	\end{array}\right] \\ \nonumber
	L_j &= \Lambda_{2,j}^{-1} (B\tran P_j(k+1) A + D W^k_{ec,j} C) \\ \nonumber 
	L_{e,j} &= \Lambda_{2,j}^{-1} D W^k_{ec,j} \\ \nonumber
	L_{w,j} &= \Lambda_{2,j}^{-1} W^k_{fc,j}, \qquad L_{g,j} = \Lambda_{2,j}^{-1} B \\ \nonumber
	\Lambda_{1,j} &= W^k_{fc,j} + W^k_{\Delta fc,j} + D\tran W^k_{ec,j} D \\ \nonumber
	\Lambda_{2,j} &= \Lambda_{1,j} + B\tran P_j(k+1) B.
\end{align} 
Matrix $P_j$ and state $g_j$ are given by the backward recursions 
\begin{align}
	P_j(k) =& H_{21,j} + H_{22,j} P(k+1) \\ \nonumber
	&(I-H_{12,j}P_j(k+1))^{-1}H_{11,j}.
\end{align}
and
\begin{align} \nonumber
	g_j(k) =& (H_{22,j}  + H_{22,j}P_j(k+1) (I-H_{12,j} P(k+1))^{-1} \\ \nonumber &  H_{12,j}) g_j(k+1) -(E_{21,j} + H_{22,j}P_j(k+1) \\ \nonumber &
	(I-H_{12,j}P(k+1))^{-1} E_{11,j}) e_j(k) -(E_{22,j} + H_{22,j} \\ 
	& P(k+1) (I-H_{12,j}P(k+1))^{-1} E_{12,j}) f_j(k)
\end{align}
where $P(N) = 0$, $g_j(N) = 0$, and
\begin{align} \nonumber 
	H_{11,j}(k) =& A(k) - B(k) \Lambda_{1,j}^{-1} D\tran(k) W^k_{ec,j} C(k) \\ \nonumber
	H_{12,j}(k) =& -B(k) \Lambda_{1,j}(k)^{-1} B\tran(k) \\ \nonumber
	H_{21,j}(k) =& C\tran(k) W^k_{ec,j} C(k) - C\tran(k) W^k_{ec,j} D(k) \\ \nonumber &\Lambda_{1,j}(k)^{-1} D\tran(k) W^k_{ec,j} C(k) \\ \nonumber
	H_{22,j}(k) =& A\tran(k) - C\tran(k) W^k_{ec,j} D(k) \Lambda_{1,j}(k)^{-1} B\tran(k) \\ \nonumber
	E_{11,j}(k) =& B(k) \Lambda_{1,j}(k)^{-1} D\tran(k) W^k_{ec,j} \\ \nonumber
	E_{12,j}(k) =& -B(k) \Lambda_{1,j}(k)^{-1} W^k_{fc,j} \\ \nonumber
	E_{21,j}(k) =& -C\tran(k) W^k_{ec,j} + C\tran(k) W^k_{ec,j} D(k) \\ \nonumber & \Lambda_{1,j}(k)^{-1} D\tran(k) W^k_{ec,j} \\ \nonumber
	E_{22,j}(k) =& -C\tran(k) W^k_{ec,j} D(k) \Lambda_{1,j}(k)^{-1} W^k_{fc,j}.
\end{align}

A similar low-order solution to ILC is also applied to the specific cases of ILC for intersample behavior in \cite{Oomen2011} and norm-optimal ILC in \cite{Zundert2016}.


\subsection{Inferential ILC considerations}
In cross-coupled ILC, the performance variables for the offline ILC computations, i.e., contour and tangential errors, differ from the online feedback variables, i.e., the individual axes errors. This leads to an inferential ILC situation which in some cases can lead to internal stability problems, see \cite{Zundert2016}. Since the current framework computes the contour errors from the individual axes errors and the coupling matrices have full column rank, it is not possible for one of the individual axes errors to blow up if the ILC system is monotonically convergent. However, opposing control actions in feedforward and feedback are possible within the framework and might be undesired. To avoid this, a serial ILC configuration, see Fig. \ref{fig:ser_ilc}, is recommended.




